BunchBFT: Across-Cluster Consensus Protocol

In this paper, we present BunchBFT Byzantine fault-tolerant state-machine replication for high performance and scalability. At the heart of BunchBFT is a novel design called the cluster-based approach that divides the replicas into clusters of replicas. By combining this cluster-based approach with hierarchical communications across clusters, piggybacking techniques for sending messages across clusters, and decentralized leader election for each cluster, BunchBFT achieves high performance and scalability. We also prove that BunchBFT satisfies the basic safety and liveness properties of Byzantine consensus. We implemented a prototype of BunchBFT in our PaxiBFT framework to show that the BunchBFT can improve the MirBFT's throughput by 10x, depending on the available bandwidth on wide-area links.

==> Akc.tex <==
\section{Acknowledgements}
This project is in part sponsored by the National Science Foundation (NSF) under award number CNS-2008243.

==> Future.tex <==
\section{Limitations and Future Work}
\label{sec:fw}
This section briefly outlines several of BigBFT2 important remaining limitations, and areas for future work.

\textbf{Evaluation of BigBFT2 with $F>0$}. A malicious leader has less effect in the overall performance. This is not the case in the Mir-BFT and other protocols, where all leaders are part of a single leaders set. Upon high rate of failures, the round-change will replace the leaders set. This will result in severe degradation in performance. In BigBFT2, failures of the leader affects the leader local region and has negligible affect on the global shards. To proof that, we need to have an evaluation of BigBFT2 under failures. 

\textbf{Future Work} Besides the issues outlined above, there are many more interesting open questions worth considering: opening up consensus group to enable permissionless Blockchian. To enable permissionless consensus by adding new leader to the consensus group that has more assignments from clients. At each round, a new leader is selected and added to the group. Every leader will hold a reputation factor known to all. Upon acting maliciously, the leader reputation goes down until the leader kicked out from the group by its trusted peers.




==> Futurework.tex <==
\section{Future Work}
\label{sec:fw}

\subsection{Improving Scalability by Enabling Local Communication}

One direction for future work is to enable hierarchical communications in order to scale the protocol to more nodes. At each round, a global coordinator selects a local coordinator in each region to maintain the configuration blockchain and to restrict the communication within each region. The global coordinator will reach consensus with local coordinators on sharding the space between regions. Local coordinator will further shard the space among all local leaders. Then, each region will run BigBFT locally among nodes to order blocks.

\subsection{Client as a Coordinator}

We are planning to enable client node to act as a system coordinator to further improve BFT scalability by reducing the interactions between replicas. The client can assign the request's sequence number, choose a set of trusted replicas to form a quorum, and learn the status of the request from the chain if committed. For instance, the client may choose a quorum of nodes including well-known validators, as shown in Stellar protocol~\cite{mazieres2015stellar}, with the high stake values to commit its blocks. Client may use blockchain to check recent honest validators that are able to commit and add to the chain. For more flexibility, the client might develop some set of policies to choose its quorum such as choosing common nodes between recent last two committed blocks. However, the system should have a security mechanism to prevent a malicious client from violating the safety of the system.
